Low-resource Neural Machine Translation with Cross-modal Alignment

How to achieve neural machine translation with limited parallel data? Existing techniques often rely on large-scale monolingual corpora, which is impractical for some low-resource languages. In this paper, we turn to connect several low-resource languages to a particular high-resource one by additional visual modality. Specifically, we propose a cross-modal contrastive learning method to learn a shared space for all languages, where both a coarse-grained sentence-level objective and a fine-grained token-level one are introduced. Experimental results and further analysis show that our method can effectively learn the cross-modal and cross-lingual alignment with a small amount of image-text pairs and achieves significant improvements over the text-only baseline under both zero-shot and few-shot scenarios.

==> Sections/100_introduction.tex <==


Machine Translation has been one of the essential tasks in natural language processing. Though with neural machine translation, the performance of the translation system is still limited by the quality and scale of parallel corpora. For low-resource languages, the insufficiency of parallel data tremendously restricts the translation accuracy.


\begin{figure}[tb]
    \centering
    \includegraphics[width=\linewidth]{figures/MMT_Figure1.pdf}
    \caption{We aim at realizing zero-shot and few-shot machine translation for the low-resource language. Different languages with the same meanings are projected to a shared space by visual-text alignment.}
    \label{fig:introduction}
\end{figure}
So how to achieve machine translation with inadequate parallel corpora becomes a hot issue. Previous studies have made some explorations. \citet{dblp1} proposed  an unsupervised machine translation method based on a large number of monolingual corpora, which is costly for low-resource languages. \citet{DBLP:conf/emnlp/LinPWQFZL20,DBLP:journals/tacl/LiuGGLEGLZ20} proposed multilingual pretraining method to achieve zero-shot translation with auxiliary parallel data of many other languages, which may cause a high cost for model training and data collection.

As \citet{ethnologue-2020} shows, there are 6,819 languages not covered by Wikipedia out of 7,097 worldwide. As a result, collecting a large amount (> 1M) of monolingual data for low-resourece language seems infeasible. However, managing a small amount (< 0.1M) of monolingual image-text pairs from social media, shopping sites, or movies is possible. In this paper, we aim to align several low-resource languages to one high-resource language with images as a pivot. We propose a cross-modal contrastive learning method to draw up the distance between text modality and visual modality. Specifically, we introduce the sentence-level and the token-level method to achieve coarse-grained and fine-grained contrastive learning, respectively. In this way, the representation of high-resource and low-resource languages with similar meanings will be brought together by the image pivot, which enables the low-resource languages to translate. As shown in Figure \ref{fig:introduction}, the high-resource language German and the low-resource language French are brought together by aligning with images, which transfer the translation ability from German to French.

% At the same time, we train a translation model on the high-resource language, then low-resource languages can achieve translation by mapping with the high-resource language. Finally, under the few-shot scenario, a few parallel corpora will be used to fine-tune the model, achieving better translation results.

In contrast with previous studies, our approach only requires a small amount of monolingual image-text pairs for the low-resource language. It provides a simple way to transfer the translation ability from the high-resource language to the low-resource language with low costs of data collection and model training. Experimental results and analysis show that: Without any parallel data, our model significantly exceeds the baseline. When with a few additional parallel data, our model still consistently outperforms the baseline with the same parallel data. 
% On zero-shot, our method achieves gains of 7.41 BLEU scores on average over the zero-shot baseline; On few-shot, our approach, with 0.01K to 0.5K parallel data, still consistently outperforms the few-shot baseline. 
Furthermore, our model can effectively realize cross-modal and cross-lingual alignment.


